Physics-Informed Induction Machine Modelling

This rapid communication devises a Neural Induction Machine (NeuIM) model, which pilots the use of physics-informed machine learning to enable AI-based electromagnetic transient simulations. The contributions are threefold: (1) a formation of NeuIM to represent the induction machine in phase domain; (2) a physics-informed neural network capable of capturing fast and slow IM dynamics even in the absence of data; and (3) a data-physics-integrated hybrid NeuIM approach which is adaptive to various levels of data availability. Extensive case studies validate the efficacy of NeuIM and in particular, its advantage over purely data-driven approaches.

==> peramble.tex <==
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{bm}
\usepackage{cases}
\usepackage{color}
\usepackage{enumitem}
\usepackage[dvipsnames]{xcolor} 
 
\usepackage[overload]{empheq}
\usepackage{graphicx}   %use graph format
\usepackage{makecell}
\usepackage{mathrsfs}
\usepackage{multirow} 
\usepackage{threeparttable} 

\usepackage{physics}    % for \dv
\usepackage{soul}

\usepackage{subcaption}
\usepackage{xspace}

\usepackage{url}
\usepackage[all]{xy}
\usepackage[font=footnotesize,labelsep=period]{caption}

%%%%%%%%%%%%%%%%%%%% tables %%%%%%%%%%%%%%%

\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}

\newcommand{\rev}[1]{{\color{blue}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{#1}


% %%%%%%%%%%%%%%% journal (default) and conference %%%%%%%%%%%%%%%
\makeatletter
\def\subsubsection{\@startsection{subsubsection}% name
                                 {3}% level
                                 {\z@}% indent (formerly \parindent)
                                 {0ex plus 0.1ex minus 0.1ex}% before skip
                                 {0ex}% after skip
                                 {\normalfont\normalsize\itshape}}% style
\makeatother

%%%%%%%%%%%%%%%%%%%% tikz %%%%%%%%%%%%%%%
\usepackage{tikz}   
\usepackage{standalone}
\usepackage{pgfplots}
\usetikzlibrary{shapes, arrows,chains,calc,shapes}
\pgfplotsset{compat = newest}
\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)





%%%%%%%%%%%%%% define the method name  %%%%%%%%%%%%%%%%%%%%%%%%
\def\insys{\textit{InSys}\xspace}
\def\exsys{\textit{ExSys}\xspace}
\def\neudyn{{NeuDyE}\xspace}
\def\odenet{{ODE-Net}\xspace}
\def\pineudyn{{PI-NeuDyE}\xspace}
\def\pgneudyn{{PG-NeuDyE}\xspace}



